FlowIE: Efficient Image Enhancement via Rectified Flow

Image enhancement holds extensive applications in real-world scenarios due to complex environments and limitations of imaging devices. Conventional methods are often constrained by their tailored models, resulting in diminished robustness when confronted with challenging degradation conditions. In response, we propose FlowIE, a simple yet highly effective flow-based image enhancement framework that estimates straight-line paths from an elementary distribution to high-quality images. Unlike previous diffusion-based methods that suffer from long-time inference, FlowIE constructs a linear many-to-one transport mapping via conditioned rectified flow. The rectification straightens the trajectories of probability transfer, accelerating inference by an order of magnitude. This design enables our FlowIE to fully exploit rich knowledge in the pre-trained diffusion model, rendering it well-suited for various real-world applications. Moreover, we devise a faster inference algorithm, inspired by Lagrange's Mean Value Theorem, harnessing midpoint tangent direction to optimize path estimation, ultimately yielding visually superior results. Thanks to these designs, our FlowIE adeptly manages a diverse range of enhancement tasks within a concise sequence of fewer than 5 steps. Our contributions are rigorously validated through comprehensive experiments on synthetic and real-world datasets, unveiling the compelling efficacy and efficiency of our proposed FlowIE. Code is available at https://github.com/EternalEvan/FlowIE.

==> figures/artifact_v2.tex <==
%\begin{table}[!h]
% \begin{wrapfigure}{r}{5cm}
\begin{wrapfigure}{r}{=0.6\linewidth}
% \centering
%\caption{\textbf{Ablation studies. Start from ${\bm\tau}_{\phi}({\bm z}_{LQ})$}
%rectified flow, mean value sampling and the first stage model.}
\vspace{-15pt}
\hspace{-2.3in}
%\adjustbox{width=\linewidth}
%{
% 

    % \begin{center}
        
    
    \includegraphics[width=\linewidth]{figures/artifact_v21.pdf}
   % \setlength{\abovecaptionskip}{5pt}
    %\caption{\textbf{Qualitative results larger resolution. }}
    
    %\vspace{-20pt}
    % \end{center}
%}

\label{fig:artifact}
\vspace{-15pt}
%\end{table}
\end{wrapfigure}

==> figures/supp_paths.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/supp_paths1.pdf}
    \caption{\textbf{The diagram of the proposed \textit{FlowIE}.} FlowIE leverages rectified flow to unleash the rich knowledge in the trained diffusion model and build straight-line paths between element distribution and clean images. The framework consistently achieves visually stunning results in a minimal number of steps and seamlessly generalizes to various image enhancement tasks, \textit{e.g.}, face inpainting, color enhancement and blind image super-resolution. }
    \label{fig:teaser}
    \vspace{-10pt}
\end{figure}

==> supp_figs/derain1.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{supp_figs/derain11.pdf}    
\end{figure*}

==> tables/bfr_main.tex <==
\begin{table*}[!t]
  \centering  
  \caption{Quantitative comparison on the \textbf{CelebA-Test}. \first{Red} and \second{blue} indicate the best and the second
best performance, respectively.}

\adjustbox{width=\linewidth}
  {\begin{tabu} to 1.2\linewidth {l*{9}{X[c]}}
    \toprule
    \multirow{3}{*}{Method} & \multirow{3}{*}{FPS$\uparrow$}& \multicolumn{5}{c}{Synthetic Dataset} & \multicolumn{3}{c}{Wild Datasets} \\
    && \multicolumn{5}{c}{CelebA} & LFW & WIDER & CelebChild \\
    %\cline{3-10}
    \cmidrule(lr){3-7}\cmidrule(lr){8-10}
     &&  PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & FID$\downarrow$ & IDS $\uparrow$ & FID$\downarrow$ & FID$\downarrow$ & FID$\downarrow$ \\
    \midrule
    GPEN~\cite{yang2021gan} &7.278& $21.3995 $ & $0.5742$ & $0.4687$ & $23.92$ & $0.48$ & $51.97$ & $46.35$ & $76.58$ \\
    GCFSR~\cite{he2022gcfsr} &10& $21.8791 $ & \grayText{\second{$0.6072$}} & $0.4577$ & $35.49$ & $0.44$ & $52.20$ & $40.86$ & $76.29$ \\
    GFPGAN~\cite{wang2021towards} &10& $21.6953 $ & \grayText{$0.6060$} & \grayText{$0.4304$} & $21.69$ & $0.49$ & $52.11$ & $41.70$ & $80.69$ \\
    VQFR~\cite{gu2022vqfr} &10& $21.3014 $ & \grayText{\first{$0.6132$}} & \grayText{\second{$0.4116$}} & \grayText{$20.30$} & $0.48$ & $49.88$ & $37.87$ & \grayText{$74.76$} \\
    RestoreFormer~\cite{wang2022restoreformer} &10 & $21.0025 $ & $0.5283$ & $0.4789$ & $43.77$ & \grayText{$0.56$} & $48.43$ & \grayText{$49.79$} & \grayText{\first{$70.54$}} \\
    DMDNet~\cite{li2022learning} &10 & $21.6617 $ & $0.6000$ & $0.4828$ & $64.79$ & \grayText{\second{$0.67$}} & \grayText{$43.36$} & $40.51$ & $79.38$ \\
    CodeFormer~\cite{zhou2022towards} &5.188 & \grayText{\first{$22.1519$}} & $0.5948$ & \grayText{\first{$0.4055$}} & $22.19$ & $0.47$ & $52.37$ & $38.78$ & $79.54$ \\
    \midrule
    DiffBIR~\cite{lin2023diffbir} &0.285 & \grayText{$21.7509$} & $0.5971$ & $0.4573$ & \grayText{\second{$20.02$}} & $0.51$ & \grayText{\second{$39.58$}} & \grayText{\second{$33.49$}} & $77.74$ \\
    \midrule
    FlowIE (Ours) &2.846 & \grayText{\second{21.9211}} & $0.6005$ & $0.4367$ & \grayText{\first{$19.81$}} & \grayText{\first{$0.68$}} & \grayText{\first{$38.66$}} & \grayText{\first{$33.41$}} & \grayText{\second{$74.25$}} \\
    \bottomrule
  \end{tabu}}
  
  \label{tab:bfr_quant}
  \vspace{-10pt}
\end{table*}



==> tables/bfr_no_gray.tex <==
\begin{table*}[!t]
  \centering  
  \caption{\textbf{Quantitative comparison on the synthetic and real-world datasets.} \first{Red} and \second{blue} indicate the best and the second
best performance, respectively. Our FlowIE shows very competitive results compared with existing methods.}
\adjustbox{width=\linewidth}
  {\begin{tabu} to 1.2\linewidth {l*{9}{X[c]}}
    \toprule
    \multirow{3}{*}{Method} & \multirow{3}{*}{FPS$\uparrow$}& \multicolumn{5}{c}{Synthetic Dataset} & \multicolumn{3}{c}{Wild Datasets} \\
    && \multicolumn{5}{c}{CelebA} & LFW & WIDER & CelebChild \\
    %\cline{3-10}
    \cmidrule(lr){3-7}\cmidrule(lr){8-10}
     &&  PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & FID$\downarrow$ & IDS $\uparrow$ & FID$\downarrow$ & FID$\downarrow$ & FID$\downarrow$ \\
    \midrule
    GPEN~\cite{yang2021gan} &7.278& $21.3995 $ & $0.5742$ & $0.4687$ & $23.92$ & $0.48$ & $51.97$ & $46.35$ & $76.58$ \\
    GCFSR~\cite{he2022gcfsr} &10& $21.8791 $ & \second{$0.6072$} & $0.4577$ & $35.49$ & $0.44$ & $52.20$ & $40.86$ & $76.29$ \\
    GFPGAN~\cite{wang2021towards} &10& $21.6953 $ & $0.6060$ & $0.4304$ & $21.69$ & $0.49$ & $52.11$ & $41.70$ & $80.69$ \\
    VQFR~\cite{gu2022vqfr} &10& $21.3014 $ & \first{$0.6132$} & \second{$0.4116$} & $20.30$ & $0.48$ & $49.88$ & $37.87$ & $74.76$ \\
    RestoreFormer~\cite{wang2022restoreformer} &10 & $21.0025 $ & $0.5283$ & $0.4789$ & $43.77$ & $0.56$ & $48.43$ & $49.79$ & \first{$70.54$} \\
    DMDNet~\cite{li2022learning} &10 & $21.6617 $ & $0.6000$ & $0.4828$ & $64.79$ & \second{$0.67$} & $43.36$ & $40.51$ & $79.38$ \\
    CodeFormer~\cite{zhou2022towards} &5.188 & \first{$22.1519$} & $0.5948$ & \first{$0.4055$} & $22.19$ & $0.47$ & $52.37$ & $38.78$ & $79.54$ \\
    \midrule
    DiffBIR~\cite{lin2023diffbir} &0.285 & $21.7509$ & $0.5971$ & $0.4573$ & \second{$20.02$} & $0.51$ & \second{$39.58$} & \second{$33.49$} & $77.74$ \\
    \midrule
    \rowcolor{gray!25}
    \Ours &2.846 & \second{21.9211} & $0.6005$ & $0.4367$ & \first{$19.81$} & \first{$0.68$} & \first{$38.66$} & \first{$33.41$} & \second{$74.25$} \\
    \bottomrule
  \end{tabu}}
  
  \label{tab:bfr_quant}
\end{table*}


